Model Consistency of Partly Smooth Regularizers

This paper studies least-square regression penalized with partly smooth convex regularizers. This class of functions is very large and versatile allowing to promote solutions conforming to some notion of low-complexity. Indeed, they force solutions of variational problems to belong to a low-dimensional manifold (the so-called model) which is stable under small perturbations of the function. This property is crucial to make the underlying low-complexity model robust to small noise. We show that a generalized "irrepresentable condition" implies stable model selection under small noise perturbations in the observations and the design matrix, when the regularization parameter is tuned proportionally to the noise level. This condition is shown to be almost a necessary condition. We then show that this condition implies model consistency of the regularized estimator. That is, with a probability tending to one as the number of measurements increases, the regularized estimator belongs to the correct low-dimensional model manifold. This work unifies and generalizes several previous ones, where model consistency is known to hold for sparse, group sparse, total variation and low-rank regularizations.

==> sections/sec-app.tex <==
% !TEX root = ../PartlySmoothSensitivity.tex

\appendix

\section{Directional Derivative and Uniqueness}
\label{sec-app}

\begin{proof}[Proof of Lemma~\ref{prop:uniqueness-directional}]
  We first show that $t \mapsto \pa{f(\x + t(z - \x)) - f(z)}/t$ is non-decreasing on $(0,1]$.
  Indeed, let $g : [0,1] \rightarrow \RR$ a convex function such that $g(0) = 0$.
  Let $(t,s) \in (0,1]^2$ with $s > t$.
  Then,
  \begin{align*}
    g(t)
    = g \pa{s (t/s)}
    &= g \pa{s (t/s) + (1 - t/s)0} \\
    &\leq t \frac{g(s)}{s} + (1 - t/s)g(0) \\
    &= t \frac{g(s)}{s} ~,
  \end{align*}
  which proves that $t \in (0,1] \mapsto \frac{g(t)}{t}$ is non-decreasing on $(0,1]$.
  Since $f$ is convex, applying this result shows that the function
  \begin{equation*}
    t \in (0,1] \mapsto g(t) = f(\x + t(z - \x)) - f(z)
  \end{equation*}
  is such that $g(0) = 0$ and $g(t)/t$ is non-decreasing.
  
  Assume now that that $f'(\x,z - \x) > 0$.
  Then, for every $\x \in C$,
  \begin{equation*}
    g(1) = f(z) - f(\x) \geq f'(\x,z - \x) > 0, \quad \forall z \in C, z \neq \x ~,
  \end{equation*}
  which is equivalent to $\x$ being the unique minimizer of $f$ on $C$.
\end{proof}



==> sections/sec-primal-dual.tex <==
% !TEX root = ../PartlySmoothSensitivity.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Primal and Dual Problems}

In this section, we do not assume that $J$ is partly smooth. We first recall some fundamental properties of both the primal and dual problems. In particular, we study the convergence of the solutions to these problems when $\la \rightarrow 0$. While these properties are not used for the proof of Theorem~\ref{thm-stability} (Section~\ref{sec-proof-thm}), they are crucial to understand the rationale behind the hypotheses of this theorem, and in particular to introduce the key concept of minimal norm certificate. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence of the Primal Problem}

We consider the following condition
\eql{\label{eq-kerPhi-kerJ}\tag{$\Ii_\Corr$}
	\ker(\Corr) \cap \ker(J_\infty) = \{0\}
	\qwhereq
	J_\infty(x) = \lim_{t \rightarrow +\infty} \frac{J(tx)}{t}
}
which is equivalent to asking that $\dotp{\Corr \cdot}{\cdot} + J$ is coercive and that 
that both problems~\eqref{eq-regularization-lagrangian} and~\eqref{eq-regularization-noiseless} have non-empty bounded sets of solutions.

We first show the convergence of the solution of the primal problem toward~$\x_0$.  

\begin{prop}\label{prop-conv-primal}
	We consider any sequence $\th_k = (\mu_k, \u_k,\Corr_k)$ where $\u_k=\Corr_k\x_0 + \epsilon_k \in \Im(\Corr_k)$. We suppose that 
	\eql{\label{eq-conve-primal}
		\pa{
			\Corr_k,
      		\frac{ \epsilon_k }{\mu_k}, 
      		\mu_k
	  	} 
		\longrightarrow 
		(\Corr,0,0), 
	}
	that $\x_0$ is the unique solution of~$(\Pp_{0,0 x_0,\CorrL})$,
	and that $(\Ii_{\CorrL})$ holds. 
	We denote $\x_k$ any solution of $(\Pp_{\th_k})$.
	Then $\x_k \longrightarrow \x_0$.
\end{prop}

\begin{proof}
	We denote $\norm{u}_\Corr^2 = \dotp{\Corr u}{u}$.
	%
	By optimality of $\x_{k}$ one has $f(\x_k,\th_k) \leq f(\x_0,\th_k)$ and hence
	\begin{align*}
		\frac{1}{2}\norm{\x_k}_{\Corr_k} - \dotp{\x_k}{\Corr_k \x_0+\epsilon_k} + \mu_k J(\x_k) 
		\leq \frac{1}{2}\norm{\x_0}_{\Corr_k} - \dotp{\x_0}{\Corr_k \x_0+\epsilon_k} + \mu_k J(\x_0)	
	\end{align*} 
	which is equivalently stated as
	\eql{\label{eq-proof-Gamma-cv-1}
		\frac{1}{2}\norm{\x_k-\x_0}_{\Corr_k}^2 - \dotp{\x_k-\x_0}{\epsilon_k} + \mu_k J(\x_k) 
		\leq
		\mu_k J(x_0).		
	}
	Since $\epsilon_k \in \Im(\Corr_k)$, we have $\epsilon_k = \Corr_k \Corr_k^+ \epsilon_k$, and hence, \eqref{eq-proof-Gamma-cv-1} implies 
	\eql{\label{eq-proof-Gamma-cv-2}
		\frac{1}{2}\norm{\x_k-\x_0}_{\Corr_k}^2 \leq \norm{\x_k-\x_0}_{\Corr_k} \norm{\Corr_k^+ \epsilon_k}_{\Corr_k} + \mu_k J(\x_0).
	}
	Since 
	\eql{\label{eq-proof-Gamma-cv-3}
		\norm{\Corr_k^+ \epsilon_k}_{\Corr_k} = \norm{\epsilon_k}_{\Corr_k^+} \leq \norm{\Corr_k^+} \norm{\epsilon_k} 
	} 
	and that $\norm{\epsilon_k} \rightarrow 0$, one has that $\norm{\Corr_k^+ \epsilon_k}_{\Corr_k}$ is bounded. Equation~\eqref{eq-proof-Gamma-cv-2} thus implies that $( \norm{\x_k-\x_0}_{\Corr_k} )_k$ is bounded.
	Similarly, \eqref{eq-proof-Gamma-cv-1} implies
	\eq{
		J(\x_k) \leq \norm{\x_k-\x_0}_{\Corr_k} \norm{\Corr_k^+ \epsilon_k/\mu_k}_{\Corr_k} + J(\x_0).
	}
	Using~\eqref{eq-proof-Gamma-cv-3} and that $\norm{\epsilon_k/\mu_k} \rightarrow 0$, one has that 
	$( \norm{\Corr_k^+ \epsilon_k/\mu_k}_{\Corr_k} )_k$ is bounded, so is $(J(\x_k))_k$. 
	%
	Hence, since 
	$\frac{1}{2}\norm{\x_k-\x_0}_{\Corr_k}^2$ and $J(\x_k)$ are bounded, thanks to condition~$(\Ii_{\CorrL})$, these bounds shows that the sequence $\{ \x_{\th_k} \}_k$ is bounded \todo{detail this since one only assume $\Ii_\Corr$ at $\Corr=\CorrL$}. We let $\x^\star$ be any accumulation point. 
	%
	Taking the limit $k \rightarrow +\infty$ in equation~\eqref{eq-proof-Gamma-cv-1} and using conditions~\eqref{eq-conve-primal} shows that $\CorrL \x^\star = \Corr \x_0$.
	%
	Furthermore, since $\frac{1}{2}\norm{\x_k-\x_0}_{\Corr_k}^2 \geq 0$, equation~\eqref{eq-proof-Gamma-cv-1} implies
	\eq{
		- \dotp{\x_k-\x_0}{\frac{\epsilon_k}{\mu_k}} +  J(\x_k) 
		\leq
		 J(x_0).		
	}
	and taking the limit $k \rightarrow +\infty$ shows that $J(\x^\star) \leq J(\x_0)$. 
	This shows that $\x^\star$ is a solution of~$(\Pp_{0,\CorrL x_0,\CorrL})$ and hence $\x^\star = \x_0$. 
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dual Problem with $(\Corr,\u)$ Variables}

The Legendre transform $J^*$ of $J$ is defined as
\eq{
	\foralls \x', \quad J^*(\x') = \umax{\x} \dotp{\x}{\x'} - J(\x). 
}

We define the dual problem, for $\th=(\mu,\u,\Corr)$ 
\eql{\label{eq-lagrangian-dual}\tag{$\Dd_\th$}
	\umin{z} g(z,\th) = 
			-\frac{\mu}{2} \dotp{\Corr z}{z} - \dotp{z}{u} 
%			- \frac{1}{2\mu} \dotp{\Corr^+ u}{u} 
			- J^*(\Corr z).
}
For any solution $z^\star$ of~\eqref{eq-lagrangian-dual}, $\eta_\th = \Corr z^\star$ is uniquely defined. 

The dual problem when $\mu=0$ reads
\eql{\label{eq-noiseless-dual}\tag{$\Dd_{\th_0}$}
	\Zz_{\th_0} = \uArgmin{z} g(z,\th) = 
		- \dotp{z}{u} - J^*(\Corr z).
} 
The following proposition states the dual problem and the primal-dual relationships.

\begin{prop}
	Assuming $\u \in \Im(\Corr)$, one has the following duality
	\eq{
		\umin{\x} f(\x,\th) = \umax{z} g(z,\th) .
	}
	For $\mu>0$, one has, for any solution $\x_\th$ of \eqref{}, 
	\eq{
		\eta_\th = \frac{ \u - \Corr \x_\th }{\mu}
		\qandq
		\eta_\th \in \partial J(\x_\th). 
	}	
	For any solution $\x_{\th_0}$ of $(\Pp_{\th_0})$, one has \todo{finish this}
	\eq{
		\Zz_{\th_0} = \ldots. 
	}
\end{prop}

\begin{proof}
	Denoting $G(\x) = \frac{1}{2\mu}\dotp{\Corr \x}{\x} - \frac{1}{\mu}\dotp{\x}{\u} + \frac{1}{2\mu}\dotp{\Corr^+ \u}{\u}$, one has
	\eq{
		G^\star(\eta) = \frac{1}{2\mu}\dotp{\Corr^+ (u + \mu \eta)}{u + \mu \eta} - \frac{1}{2\mu}\dotp{\Corr^+ \u}{\u} + \iota_{\Im(\Corr)}(\u + \mu \eta).
	}	
	One verifies that strong duality holds and allows to write $\min G+J = \max -G^*-J^*$. Since by hypothesis $\u \in \Im(\Corr)$, constraint $\u + \mu \eta \in \Im(\Corr)$ can be re-written as $\eta \in \Im(\Corr)$, and thus we introduce $\eta = \Corr z$ and consider 
	\eq{
		\umin{\x} f(\x,\th) = \umax{z} 
		- \frac{1}{2\mu}\dotp{\Corr^+ (u + \mu \Corr z)}{u + \mu \Corr z} + \frac{1}{2\mu}\dotp{\Corr^+ \u}{\u} - J^*( \Corr z ), 
	}
	which is the desired expression. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dual Problem with $(\Phi,y)$ Variables}


For $\la>0$, the Fenchel-Rockafellar dual problem associated to~\eqref{eq-regularization-lagrangian} reads
\eql{\label{eq-lagrangian-dual}\tag{$\Dd_\th$}
	\p_\th = \uargmin{\p \in \RR^\P}
	g(\p, \th) = J^*(\Phi^* \p)  - \dotp{y}{\p} + \frac{\la}{2} \norm{\p}^2.
}
Note that $\p_\th$ is uniquely defined because $g(\cdot,\th)$ is strictly convex. 

\todo{These dual variables $\al$ are related to the previous variable $z$ by $\Phi^*\al=\Corr z$ and  $\Phi z = \al$. }

The following proposition recalls the primal-dual relationships.

\begin{prop}\label{prop-primal-dual}
	For any solution $\x_\th$ of~\eqref{eq-regularization-lagrangian}, one has
	\eq{
		\p_\th = \frac{ y - \Phi^* \x_\th }{\la}
		\qandq
		\eta_\th = \Phi^* \p_\th \in \partial J(\x_\th).
	}
\end{prop}
\begin{proof}
	Since $J$ is convex and has full domain, strong duality holds, hence the result using Fenchel-Rockafellar duality. 
\end{proof}

For $\la=0$, the dual problem associated to~\eqref{eq-regularization-noiseless} reads
\eql{\label{eq-noiseless-dual}\tag{$\Dd_{\th_0}$}
	\Ss_{\th_0} = \uArgmin{\p \in \RR^\P}
	g(\p, \th_0) = J^*(\Phi^* \p) - \dotp{y}{\p}.
}
Note that in general $\Ss_{\th_0}$ is not a singleton. The following proposition shows how $\Ss_{\th_0}$ relates to solution of the primal problem.

\begin{prop}\label{prop-primal-dual-constraint}
	For any solution $\x_{\th_0}$ of $(\Pp_{\th_0})$, one has
	\eq{
		\Ss_{\th_0} = \enscond{\p \in \RR^\P}{ \Phi^* \p \in \partial J(\x_{\th_0}) }. 
	}
\end{prop}
\begin{proof}
	Similarly to Proposition~\ref{prop-primal-dual}, strong duality holds between 
	$(\Pp_{\th_0})$ and $(\Dd_{\th_0})$, and the primal-dual relationships states that 
	$(\x_{\th_0},\p_{\th_0})$ form a solution to these problems if and only if $\Phi^* \p_{\th_0} \in \partial J(\x_{\th_0})$.
\end{proof}

Note that $p_{\th_0}$ is well defined because it is the projection of $0$ on the closed convex set $\Ss_{\th_0}$. In the following, we make use of the following notations
\eq{
	\p_0 = \p_{\th_0^0}
	\qandq
	\eta_0 = \Phi^* \p_0.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence of the Dual Problem}

The following definition singles out a particular solution of the dual problem.

\begin{defn}[Minimal norm certificate] We define
\eql{\label{eq-min-norm-certif}
	\tetaL{\Corr} = \Corr \uArgmin{z \in \Zz_{\th_0^0}} \dotp{\Corr z}{z}.
}
which can be shown to be uniquely defined \todo{detail why}. 
\end{defn}

The following proposition gives the limit of $\eta_\th$ for small $\mu$ and $\epsilon$.

\begin{prop}\label{prop-conv-dual}
	Under the same hypothesis as \eqref{prop-conv-primal}, one has
	\eq{
		\eta_{\th_k} \rightarrow  \tetaL{\Corr}.
	}
\end{prop}
\begin{proof}
	\todo{}
\end{proof}

\if 0 %%% OLD %%%
\begin{prop}\label{prop-conv-dual}
We consider 
One has 
\eq{
	\norm{ \p_\th - \p_0 } \leq  \frac{\norm{y-y_0}}{\la} + \epsilon(\la)
}
where $\epsilon(\la) \rightarrow 0$ when $\la \rightarrow 0$. 
\end{prop}
\begin{proof}
	This result is already proved in~\cite{2013-duval-sparsespikes} in a special case of functional $J$.
	%
	Formulation~\eqref{eq-lagrangian-dual} shows $\p_\th$ is the proximal operator of the function $J^*(\Phi^* \cdot)/\la$ applied at the point $y/\la$. This shows that $y/\la \mapsto \p_\th$ is 1-Lipschitz, and hence
	\eq{
		\norm{\p_\th - \p_0 } \leq 
		\norm{\p_\th - \p_{(\la,y_0,\Phi)}} + \norm{\p_{(\la,y_0,\Phi)} - \p_0} 
		\leq 		
		\frac{\norm{w}}{\la} + \norm{\p_{(\la,y_0,\Phi)} - \p_0 }.
	}
	We now prove that 
	\eq{
		\p_\th \overset{\la \rightarrow 0}{\longrightarrow} \p_{\th_0},
	}
	which gives the desired result when setting $y=y_0$ in the previous formula. 
	
	
	Since $\p_{\th_0}$ is a solution of~\eqref{eq-noiseless-dual}, one has
	\eql{\label{eq-dual-proof-1}
		-\dotp{\p_{\th_0}}{y} \leq -\dotp{\p_\th}{y}.
	}
	By optimality of $\p_\th$, one has $g(\p_\th,\th) \leq g(\p_{\th_0},\th)$, and thus
	\eq{
		-2\dotp{\p_\th}{y} + \la \norm{\p_\th}^2 
		\leq 
		-2\dotp{\p_{\th_0}}{y} + \la \norm{\p_{\th_0}}^2
		\leq 
		-2\dotp{\p_\th}{y} + \la \norm{\p_{\th_0}}^2	 
	}
	and thus
	\eql{\label{eq-dual-proof-2}
		\norm{\p_\th} \leq \norm{\p_{\th_0}}.
	}
	This shows that $\{ \p_\th \}_{\la}$ is bounded. Let $\p^\star$ be any cluster point. 
	Operating as in the proof of Proposition~\ref{prop-conv-primal}, we have $\foralls \bar{\x} \in \enscond{\x}{y=\Phi \x}$
	\begin{align*}
		\norm{ y - \Phi \x_\th }^2 \leq 2\la J(\bar{\x}) \qandq J(\x_\th) \leq J(\bar{\x}). 
	\end{align*} 
	Letting $\lambda \to 0$, we get by continuity that
	\eq{
		\x_{\th_0} \in \enscond{\x}{y=\Phi \x} \qandq J(\x_\th) \leq J(\bar{\x}) ~,
	}
	or equivalently, that $\x_{\th_0}$ is a minimizer of \eqref{eq-regularization-noiseless}.
	Morever, from the primal-dual extremality relationships, we have $\Phi^* \p_\th \in \partial J(\x_\th)$. Since $J$ is a proper closed convex function, the graph of $\partial J$ is sequentially closed, which yields $\Phi^* \p^\star \in \partial J(\x_{\th_0})$, i.e. $\p^\star \in \Ss_{\th_0}$.
	Now~\eqref{eq-dual-proof-2} implies that $\norm{\p^\star} \leq \norm{\p_{\th_0}}$ and hence $\p^\star=\p_{\th_0}$, which shows that $\p_\th$ is converging to $\p_{\th_0}$.
\end{proof} 
\fi %%% END OLD %%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uniqueness Sufficient Conditions}

% The following result is the extension of a classical result from $\ell^1$ minimization to arbitrary $J$ functionals, see for instance~\cite{fuchs2004on-sp}. 

Proposition~\ref{prop:uniqueness} below follows the strategy of proof already used in~\cite{vaiter2013model}. However, to simplify the exposition of the proof, we assume that $J$ is partly smooth at $\x_\th$ a solution of~\eqref{eq-regularization-lagrangian}. We start by the following lemma.

\begin{lem}\label{prop:uniqueness-directional}
  Let $C$ be a non-empty closed convex set and $f$ a proper lsc convex function.
  Let $\x$ be a solution of $\min_{z \in C} f(z)$.
  If
  \begin{equation*}
		f'(\x,z - \x) > 0 \quad \foralls z \in C, z \neq \x ~, 
  \end{equation*}
  then, $\x$ is the unique solution of $f$ on $C$.
\end{lem}

\begin{proof}
  One first check that the function $t \mapsto \pa{f(\x + t(z - \x)) - f(z)}/t$ is non-decreasing on $(0,1]$.  
  Assume now that that $f'(\x,z - \x) > 0$.
  Then, for every $\x \in C$,
  \begin{equation*}
    g(1) = f(z) - f(\x) \geq f'(\x,z - \x) > 0, \quad \foralls z \in C, z \neq \x ~,
  \end{equation*}
  which is equivalent to $\x$ being the unique minimizer of $f$ on $C$.
\end{proof}

We now state the uniqueness result.

\begin{prop}\label{prop:uniqueness}
  	Let $\x_\th$ be a solution of~\eqref{eq-regularization-lagrangian} (resp. a feasible point of~\eqref{eq-regularization-noiseless}).
  	Assume that there exists $\p$ such that $\eta = \Corr \p \in \ri( \partial J(\x_\th) )$, and such that
  \begin{equation*}
    	\ker(\Corr) \cap T = \{0\}, 
  \end{equation*}
  where $T = T_{\x}$.
  Assume also that $J$ is partly smooth at $\x_\th$ relative to the manifold $\Mm$.
  Then $\x_\th$ is the unique solution of~\eqref{eq-regularization-lagrangian} (resp.~\eqref{eq-regularization-noiseless}).
\end{prop}
\begin{proof}
  	One has
  	\begin{equation*}
    \eta \in \ri(\partial J(\x_\th))
    \Leftrightarrow
    	J'(\x_\th,\delta) > \dotp{\eta}{\delta} \quad \foralls \delta  \text{ such that } J'(\x_\th,\delta) + J'(\x_\th,-\delta) > 0 .
  	\end{equation*}
  	Applying this with $\eta = \Corr \p \in \ri(\partial J(\x_\th))$, we obtain
  	\begin{equation*}
    	\Corr \p \in \ri(\partial J(\x_\th))
    	\Leftrightarrow
    	J'(\x_\th,\delta) > \dotp{\p}{\Corr \delta} \quad \foralls \delta  \text{ such that } 
    	J'(\x_\th,\delta) + J'(\x_\th,-\delta) > 0 .    
  	\end{equation*}
  	Now, since $J$ is sharp (Definition~\ref{dfn-partly-smooth}, (ii)) at $\x$, using~\cite[Proposition 2.4]{Lewis-PartlySmooth}, we have
  	\begin{equation*}
     	J'(\x_\th,-\delta) > J'(\x_\th,\delta)
     	\qforq
     	\foralls \delta \in N_\Mm(\x_\th) \setminus \ens{0} .
  	\end{equation*}
  	Hence,
  	\begin{equation*}
    	\Corr \p \in \ri(\partial J(\x_\th))
    	\Rightarrow
    	J'(\x_\th,\delta) > \dotp{\p}{\Corr \delta} \quad \foralls \delta \in N_\Mm(\x_\th) \setminus 			\ens{0}.
  	\end{equation*}
  	Since $N_\Mm(\x_\th) = T_{\x}^\bot$, we have
  	\begin{equation*}
    	\Corr \p \in \ri(\partial J(\x_\th))
    	\Rightarrow
    	J'(\x_\th,\delta) > 0 \quad \foralls \delta \in \Ker \Corr \setminus \ens{0},
  	\end{equation*}  
  	which concludes the proof using Lemma~\ref{prop:uniqueness-directional}.
\end{proof}

The following proposition explains the connexion between $\etaL{\Corr}$ and the minimal norm certificate. 

\begin{prop}\label{prop-uniqueness}
       Suppose $J$ is partly smooth at $\x_0$ for the manifold $\Mm$.
	Under the hypothesis $\ker(\Corr) \cap T = \{0\}$, one has
	\begin{align}
	\label{eq-prop-uniqueness-1}
		\etaL{\Corr} \in \ri(\partial J(\x_0))
		&\quad\Longrightarrow\quad
			\tetaL{\Corr} = \etaL{\Corr}, \\
			\label{eq-prop-uniqueness-2}
		\tetaL{\Corr} \in \ri(\partial J(\x_0))
		&\quad\Longrightarrow\quad
		\tetaL{\Corr} = \etaL{\Corr}.
	\end{align}
	These conditions implies that $\x_0$ is the unique solution of $(\Pp_{\th_0^0})$.
\end{prop}
\begin{proof}
	\todo{Needs re-writing with the new notations.}
	We first remark that the first order condition of $(\Pp_{\th_0^0})$ reads
	\eq{
		\x_0 \text{ solution of } (\Pp_{\th_0^0})
		\Longleftrightarrow 
		\exists \eta \in \Im(\Phi^*) \cap \partial J(\x_0).
	}	
	This shows that the left hand side conditions of both~\eqref{eq-prop-uniqueness-1} and~\eqref{eq-prop-uniqueness-2} implies that $\x_0$ is a solution of $(\Pp_{\th_0^0})$. 
	
	\smallskip\noindent\textit{Proof of~\eqref{eq-prop-uniqueness-1}} 
		Under the condition $\ker(\Phi) \cap T = \{0\}$, one has, from the definition of $\Phi_T^{*,+}$, that 
		\eql{\label{eq-pf-variational}
			\pF = \uargmin{\p} \enscond{ \norm{\p} }{ \Phi_T^* \p = e }
		}
		
		Using Proposition~\ref{prop-primal-dual-constraint} for $w=0$ with $\x_0$ being solution of $(\Pp_{\th_0^0})$, one sees that the constraint of problem~\eqref{eq-pf-variational} includes the constraint of problem~\eqref{eq-min-norm-certif}. Indeed, one has
		\eq{
			\foralls \eta \in \partial J(\x), \quad P_{T_{\x}}(\eta) = e_{\x}.
		}
		
		If $\pF \in \ri(\partial J(\x_0))$, then it is a feasible point of problem~\eqref{eq-min-norm-certif} when $w=0$. Hence, necessarily $\p_0=\pF$.

	\smallskip\noindent\textit{Proof of~\eqref{eq-prop-uniqueness-2}} Since $\x_0$ is a solution of $(\Pp_{\th_0^0})$, according to Proposition~\ref{prop-primal-dual-constraint}, one has that 
	\eq{
		\p_0 = \uargmin{\p} \enscond{\norm{\p}^2}{ \Phi_T^* \p = e, \Phi_S^* \p \in \Uu  }
	}
	where we have denoted $S=T^\bot$ and $\Uu = P_S( \partial J(\x_0) )$. The first order conditions of this problem state the existence of $q \in \RR^\N$ and $u \in \RR^\N$ such that
	\eq{
		\p_0 + \Phi_T q + \Phi_S u  = 0 \qwhereq
		\choice{
			\Phi_T^* \p_0 = e, \\
			u \in \Nn_{\Uu}(\Phi_S^* \p_0).
		} 
	}
	The condition $\Phi^* \p_0 \in \ri(\partial J(\x_0))$ implies that $\Phi_S^* \p_0 \in \ri(\Uu)$ and thus $\Nn_{\Uu}(\Phi_S^* \p_0) = T$. This implies $\Phi_S u = 0$ and hence one has the equation
	\eq{
		\Phi_T^* \p_0+ \Phi_T^* \Phi_T  q =  e + \Phi_T^* \Phi_T  q = 0	
	}
	which leads to $\p_0 = (\Phi_T)^{+,*} e = \pF$.
	
	\smallskip\noindent\textit{Proof of uniqueness.} 
	See Proposition~\ref{prop:uniqueness}.
\end{proof}



